NeFF-BioNet: Crop Biomass Prediction from Point Cloud to Drone Imagery

Crop biomass offers crucial insights into plant health and yield, making it essential for crop science, farming systems, and agricultural research. However, current measurement methods, which are labor-intensive, destructive, and imprecise, hinder large-scale quantification of this trait. To address this limitation, we present a biomass prediction network (BioNet), designed for adaptation across different data modalities, including point clouds and drone imagery. Our BioNet, utilizing a sparse 3D convolutional neural network (CNN) and a transformer-based prediction module, processes point clouds and other 3D data representations to predict biomass. To further extend BioNet for drone imagery, we integrate a neural feature field (NeFF) module, enabling 3D structure reconstruction and the transformation of 2D semantic features from vision foundation models into the corresponding 3D surfaces. For the point cloud modality, BioNet demonstrates superior performance on two public datasets, with an approximate 6.1% relative improvement (RI) over the state-of-the-art. In the RGB image modality, the combination of BioNet and NeFF achieves a 7.9% RI. Additionally, the NeFF-based approach utilizes inexpensive, portable drone-mounted cameras, providing a scalable solution for large field applications.

==> sec/0_abstract_7_Sep.tex <==
\begin{abstract}
Crop biomass provides insightful information relating to plant growth, health, and productivity and as such is valuable for crop breeding programs and agronomic research. However, this trait cannot currently be quantified at scale due to the limitations of existing measurement methods, characterised by labour-intensive, destructive, and approximate measurement. To tackle this issue, we propose a generalized biomass prediction network (generalized BioNet) that can be easily adapted to multiple modalities, such as images and point clouds. Our generalized BioNet, comprising a sparse 3D convolutional neural network (CNN) and a transformer-base prediction module, takes the point cloud or other 3D data representations as input to predict biomass. To generalize BioNet for multi-view images, we introduce a neural feature field (NeFF) module, which can reconstruct the 3D structure and distill 2D semantic feature maps from the vision foundation model into the corresponding 3D surface. For the point cloud modality, our BioNet is evaluated on two public datasets and it outperforms the current state-of-the-art method by at least approximately 6.1\% relative improvement (RI). For the RGB imagery modality, we combine the NeFF and BioNet, which shows a 9.8\% RI. Moreover, the method, consisting of NeFF and BioNet, relies on ubiquitous, portable, and inexpensive cameras mounted on a drone and as such presents the advantage of being scalable to large fields.
\end{abstract}

==> sec/1_intro_7_Sep.tex <==
\vspace*{-\baselineskip}

\section{Introduction}
\label{sec:intro}

The amount of organic matter a plant produces is called biomass. Biomass estimation and mapping at large scale (up to global maps) is widely studied in the remote sensing community~\cite{DUNCANSON2022112845, bullock2023estimating}. Such large-scale biomass estimates are carried out at resolutions ranging between 30~m to 1~km, predominately for vegetation (e.g. forest) biomass. In this paper, we focus on crop biomass estimation at high resolution (i.e. sub meter-scale), where the term `biomass' specifically refers to above-ground biomass (ie. excluding roots). Crop biomass is a key trait to monitor in agricultural systems. It is used to determine the rate of plant establishment to inform decisions around replanting or to apply a range of management measures such as chemical sprays. It is also a parameter to determine which test lines to select in crop breeding programs. Unfortunately, measuring this trait at scale is currently impractical due to the limitations of existing methods \cite{pan2022biomass, loudermilk2009ground}. 


Conventional biomass quantification relies on harvesting and measuring the biomass of a small plot area (eg. a square meter or a linear meter) and relating this value to a whole plot or field. This approach is a destructive and laborious approximation, which means that it does not scale and cannot be used to generate temporal data. On the contrary, computer vision offers the opportunity to non-destructively measure biomass through time \cite{walter2019estimating, jimenez2018high, caballer2021prediction, sun2018field, polo2009tractor, ten2019biomass, pan2022biomass}.  LiDAR in particular has been used to capture plant height and point density, serving as a proxy to estimate biomass.  Proxy-based methods tend to be generalizable, but their simple 3D feature representation and canopy self-occlusion limit their accuracy. To further improve estimation accuracy, deep learning mechanisms have been introduced to address the issue of self-occlusion and learn strong 3D features from point clouds~\cite{pan2022biomass, li2024mmcbe}. However, current deep learning-based methods still suffer from low accuracy due to the difficulty of extracting 3D features, and limited availability of relevant and sizeable training datasets. To overcome these issues, we propose a generalized biomass backbone network, mainly comprising sparse 3D CNN operations on point clouds. This network inherently benefits from translation invariance and parameter sharing and reduction~\cite{NIPS2012_c399862d, lecun1998gradient}, improving generalization beyond small datasets. Since the sparse 3D CNN mainly focuses on the exploitation of local structures, we further enhance the model by incorporating an attention mechanism (Transformer encoders~\cite{vaswani2017attention}) to extract the global feature from 3D CNN feature maps for the final biomass prediction, as shown in ~\cref{fig:overal_framework}. Our generalized BioNet is evaluated on two public biomass datasets~\cite{pan2022biomass, li2024mmcbe}. The experimental results demonstrate superior prediction accuracy and stronger generalization capability compared to the state-of-the-art (SOTA).

The requirement for high-resolution LiDAR point cloud data could constrain the scalability of our approach to large fields. In comparison, vision-based biomass measurement methods (i.e. those relying on RGB imaging) are particularly appealing due to the widespread availability and affordability of RGB cameras. To adapt the generalized BioNet to images, we introduce a NeFF module to extract 3D feature maps from multi-view images, using neural implicit fields to learn the geometry, radiance, and semantic features of crops. Specifically, NeFF reconstructs 3D crops from the neural geometry field and scatters semantic features from the learned feature field to the reconstructed 3D crop surfaces. Subsequently, our generalized BioNet takes the extracted 3D features as input for final biomass prediction. Experimental results demonstrate that our BioNet with NeFF achieves about 9.8\% accuracy gains over the SOTA methods. This vision and learning-based approach to biomass estimation holds potential for large-scale application. Our key contributions are summarized as follows:
\begin{itemize}
    \item We have proposed a new 3D backbone network that consists of sparse 3D CNN and Transformer encoder, demonstrating better prediction accuracy and stronger generalization capability than the SOTA;
    \item We have developed an implicit neural network that can generate 3D feature maps from multi-view images, its combination with our generalized BioNet can achieve higher prediction accuracy compared to other vision-based biomass measurement methods and has the potential to scale to large fields;
    \item We have conducted extensive experiments using public datasets, which include both evaluation and ablation studies.
\end{itemize}

%1). we have proposed a new 3D backbone network that consists of sparse 3D CNN and Transformer encoder, demonstrating better prediction accuracy and stronger generalization capability than the SOTA; 2). we have developed an implicit neural network that can generate 3D feature maps from multi-view images, its combination with our generalized BioNet can achieve higher prediction accuracy compared to other vision-based biomass measurement methods and has the potential to scale to large fields; 3). we have conducted extensive experiments using public datasets, which include both evaluation and ablation studies.

\noindent In this paper, we present related work in~\cref{sec:related_work}, followed by the introduction of our approach in~\cref{sec:BPN} and~\cref{sec:NeFF}. We conduct extensive experimental studies in~\cref{sec:experiments}, and conclude the paper with~\cref{sec:conclusion}.


==> sec/3_method_simplied_gpt.tex <==
\section{Generalized BioNet}\label{sec:BPN}
\vspace*{-0.2cm}

Given a 3D input, which can be either point cloud or 3D feature maps, denoted as ${\boldsymbol{P}} \in \mathbb{R}^{n \times (3+f)}$, where $n$ is the number of points, 3 represents the spatial coordinates, and $f$ is the point feature channel (e.g., $f=3$ for colorized point clouds), the generalized BioNet processes ${\boldsymbol{P}}$ to predict biomass. Since the 3D structure of crops is closely correlated with biomass, we employ sparse 3D CNNs to extract 3D local features from ${\boldsymbol{P}}$. Sparse 3D CNNs are chosen for their efficiency in terms of fewer learning parameters and translation invariance, outperforming MLP and Transformer in these respects. We further incorporate Transformer networks\cite{vaswani2017attention, dosovitskiy2020image, chen2021crossvit} to capture global features for robust biomass prediction. The hybrid architecture of generalized BioNet is shown in\cref{fig:bpn}.

\subsection{3D Feature Extraction}
The 3D input $\boldsymbol{P}$ typically contains sparse geometrical data, so we design a backbone network (denoted as $\mathcal{H}(.)$) based on sparse 3D CNN layers to extract the 3D geometric features $\boldsymbol{f}^{3D}$, as expressed in~\cref{equ:3dcnn}. Sparse 3D CNNs leverage spatial sparsity to reduce memory usage and processing costs while requiring fewer parameters~\cite{s18103337}. Since sparse 3D CNNs expect the input $\boldsymbol{P}$ to be on a regular grid, we first voxelize the point cloud to generate voxel-based representations. Each voxel is populated by averaging the features of points it contains. This yields a high-resolution voxelized feature map with dimensions $c \times h \times w \times h$, where $c=(3+f)$. Typically, $h$ (height) is the smallest dimension as crop height tends to be less than plot width and length. The 3D features are then processed through sparse 3D CNN blocks, using a $3 \times 3 \times 3$ convolutional kernel and submanifold CNN~\cite{graham2017submanifold} until the height dimension collapses, resulting in a 2D feature map $\boldsymbol{f}^{3D} \in \mathbb{R}^{h^t \times w^t \times c^t}$. The full architecture is detailed in the supplementary material.
\begin{equation}
\boldsymbol{f}^{3D} = \mathcal{H}(\boldsymbol{P})
\label{equ:3dcnn}
\end{equation}

\subsection{Transformer for Biomass Prediction}
The Transformer architecture has proven highly effective in computer vision tasks\cite{carion2020end, dosovitskiy2020image, misra2021end, vaswani2017attention}, making it an ideal choice for biomass prediction. After extracting the feature map $\boldsymbol{f}^{3D}$ from the sparse 3D CNN, we flatten it into a 1D token sequence $\boldsymbol{f}^{3D}_{t} \in \mathbb{R}^{(h^t\times w^t) \times c^t}$. We introduce a learnable \texttt{Biomass} token, similar to the \texttt{Class} token in Vision Transformers (ViT)\cite{dosovitskiy2020image}, which serves as a representative embedding for the 3D feature map. This \texttt{Biomass} token interacts with spatial features and summarizes the overall scene. Positional embeddings are also added to retain spatial information. The final sequence of embedding vectors is passed through Transformer encoders, and a biomass prediction head (two-layer MLP) is connected to the \texttt{Biomass} token to predict the final biomass value $\hat{m}$:
\begin{equation}
\hat{m} = \mathcal{F}(\boldsymbol{f}^{3D}_{t})
\label{equ:trans}
\end{equation}

Given the ground truth biomass $m_i$, we compute the biomass prediction loss as follows:
\begin{equation}
\begin{aligned}
\mathcal{L}{b} =  \sum{i=1}^{N} \boldsymbol\ell1\left( \frac{\hat{m}_i - m_i}{\log(m_i)} \right)
\label{equ:bio_pred}
\end{aligned}
\end{equation}
\noindent where $\boldsymbol\ell1$ represents the smooth L1 loss function\cite{smoothl1}. We regularize the error between prediction and ground truth using $\log(m_i)$ to ensure the loss function is more sensitive to smaller biomass values. Thus, prediction errors are penalized less as biomass increases. The relationship between prediction error and regularized error is illustrated in\cref{fig:loss}.

\section{Neural Feature Field}
\label{sec:NeFF}

Vision-based biomass prediction is particularly appealing due to the widespread availability of RGB cameras. To extend BioNet to vision systems, we introduce a Neural Feature Field (NeFF) that extracts 3D features from drone images. Given multi-view images of a static scene $(I_{1}, I_{2}, \ldots, I_{n})$, $I_i \in \mathbb{R}^{3 \times H \times W}$, NeFF distills 2D features from foundation models into a 3D representation suitable for biomass prediction. These 3D features encode both semantic content and 3D spatial structure, aiding in crop differentiation and isolation from the ground.

\subsection{Neural Implicit Scene Representation}
A scene’s representation consists of two main aspects: geometry and appearance. Similar to NeuS\cite{NeuS_3D_reconstru}, we represent scene geometry using a Signed Distance Function (SDF) to capture 3D structures and decouple geometry from appearance information\cite{yariv2020multiview, NeuS_3D_reconstru, yariv2021volume}. The geometry function $\mathcal{E}{g}$ maps a 3D location $\textit{\textbf{x}} = (x,y,z) \in \mathbb{R}^{3}$ to its signed distance $s \in \mathbb{R}$:
\begin{equation}
\begin{aligned}
\textit{S} = { \textbf{\textit{x}} \in \mathbb{R}^{3} | \mathcal{E}{g}(\textbf{\textit{x}}) = 0 }
\label{equ:sdf}
\end{aligned}
\end{equation}

The appearance (radiance) field, represented by $\mathcal{E}{c}$, maps a point’s position $\mathbf{x}$ and viewing direction $\mathbf{v} \in \mathbb{R}^{2}$ to the emitted color $\mathbf{c} \in \mathbb{R}^{3}$ (RGB). Using volume rendering, the expected color along a ray $\mathbf{r}$ is computed as:
\begin{equation}
\begin{aligned}
\mathbf{\hat{c}(r)} =  \int{t_{\text{n}}}^{t_{\text{f}}} w(t)\mathcal{E}_{c}(\mathbf{x}(t), \mathbf{v})dt
\label{equ:volume}
\end{aligned}
\end{equation}

\subsection{Semantic Feature Representation}
\label{sec:feature_field_rep}
To generate a continuous 3D semantic feature volume, NeFF distills knowledge from the 2D DINO foundation model~\cite{caron2021emerging}, which has strong generalization capabilities. The mapping function for the semantic feature field is $\mathcal{E}{f}: \mathbf{x} \longrightarrow \mathbf{f}$, where $\mathbf{f} \in \mathbb{R}^{c}$ is the feature vector. Similar to color rendering, the 2D feature map can be represented as:
\begin{equation}
\begin{aligned}
\mathbf{\hat{f}(r)} = \int{t_{\text{n}}}^{t_{\text{f}}} w(t)\mathcal{E}_{f}(\mathbf{x}(t))dt
\label{equ:feature}
\end{aligned}
\end{equation}

Once $\mathcal{E}{f}$ is learned, the **3D semantic feature $F{3D}$** can be extracted by inputting surface points $\textit{S}$:
\vspace*{-0.2cm}
\begin{equation}
